Deep Hedging: Learning to Simulate Equity Option Markets

We construct realistic equity option market simulators based on generative adversarial networks (GANs). We consider recurrent and temporal convolutional architectures, and assess the impact of state compression. Option market simulators are highly relevant because they allow us to extend the limited real-world data sets available for the training and evaluation of option trading strategies. We show that network-based generators outperform classical methods on a range of benchmark metrics, and adversarial training achieves the best performance. Our work demonstrates for the first time that GANs can be successfully applied to the task of generating multivariate financial time series.

==> table_full_path.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{3}{c}{Distributional} & \multicolumn{2}{c}{Dependence} &  \multicolumn{2}{c}{Cross-Correlation} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Models  & \multicolumn{1}{l}{$|\hat f_h(B) - \hat f_r(B)|$} & \multicolumn{1}{l}{skew} & \multicolumn{1}{l}{kurtosis} & \multicolumn{1}{l}{$\operatorname{ACF}^X(16)$} & \multicolumn{1}{l}{$\operatorname{ACF}^R(1)$} & \multicolumn{1}{l}{$\| \hat \Sigma^X_h - \hat \Sigma^X_g \|_2$} & \multicolumn{1}{l}{$\| \hat \Sigma^R_h - \hat \Sigma^R_g \|_2$} \\
\bottomrule
VAR(2)                        & 0,100      & 0,443    & 0,435    & 0,636      & \textbf{0,042}     & 4,955                    & 10,322  \\
VAR(2) - PCA(5)       & 0,217      & 0,448    & 7,968    & 0,674      & 0,045     & 1,121                    & 7,968     \\
qMLE                  & 0,108                                                                  & 0,570                                         & 0,762                                             & 1,054                                                              & 0,204                                                           & 4,986                                                                                & 17,658                                                                               \\
qMLE - PCA(5) & 0,069                                                                  & 0,410                                         & 0,501                                             & 1,110                                                              & 0,069                                                           & 5,559                                                                                & 4,496                                                                                \\
GAN                           & \textbf{0,030}                                                                  & \textbf{0,087}                                         & \textbf{0,229}                                             & \textbf{0,202}                                                              & 0,092                                                           & \textbf{0,903}                                                                               & 5,054                                                                                \\
GAN - PCA(5)          & 0,037                                                                  & 0,240                                         & 0,559                                             & 0,367                                                              & 0,074                                                           & 2,014                                                                                & 4,377                                                                                \\
WGAN                          & 0,038                                                                  & 0,221                                         & 0,861                                             & 0,328                                                              & 0,062                                                           & 1,565                                                                                & 4,861                                                                                \\
WGAN - PCA(5)        & 0,043                                                                  & 0,219                                         & 0,332                                             & 0,209                                                              & 0,074                                                           & 1,325                                                                                & \textbf{4,376}                                                                               \\
%\bottomrule
%Lower Bound Compression       & 0,025      & 0,088    & 0,232    & 0,146      & 0,036     & 1,191                    & 4,722 \\
\bottomrule
\end{tabular}}
\captionof{table}{Numerical results obtained by using the full historical path.}
\label{table:full_path}
\end{table}


